Multi-Category Fairness in Sponsored Search Auctions

Fairness in advertising is a topic of particular concern motivated by theoretical and empirical observations in both the computer science and economics literature. We examine the problem of fairness in advertising for general purpose platforms that service advertisers from many different categories. First, we propose inter-category and intra-category fairness desiderata that take inspiration from individual fairness and envy-freeness. Second, we investigate the "platform utility" (a proxy for the quality of the allocation) achievable by mechanisms satisfying these desiderata. More specifically, we compare the utility of fair mechanisms against the unfair optimal, and we show by construction that our fairness desiderata are compatible with utility. That is, we construct a family of fair mechanisms with high utility that perform close to optimally within a class of fair mechanisms. Our mechanisms also enjoy nice implementation properties including metric-obliviousness, which allows the platform to produce fair allocations without needing to know the specifics of the fairness requirements.

==> sections/lowerbounds.tex <==
Let's suppose that we have a general function of the bids $F$ (using notation from Section 4.2). What kind of upper bounds on the fair value can we obtain? We ideally want to show an upper bound that decays with $k$ to show that the proportional allocation style dependence is optimal. That is, we want to show that to maintain a fixed fair value, the bid ratio condition must become stronger as the number of advertisers grows.

If we have only two types of bids $B_{high}, B_{low}$, the upper bounds with uniform metrics will not look very good, where $B_{high} = \alpha$. The allocation will have to be some function of the number of high bids. We know that $B_{low}, B_{low}, \ldots, B_{low}$ will be $\frac{1}{k}, \ldots, \frac{1}{k}$. Imagine a mechanism that does the following: if there are $H$ advertiser who bid $B_{high}$, then the mechanism places $\frac{1}{k} + \frac{d(k-H)}{Hk}$ on $B_{high}$ and places a $\frac{1}{k} - \frac{d}{k}$ on $B_{low}$. This mechanism seems to satisfy total variation fairness on these bids. This mechanism will achieve a fair value of $\frac{H}{k} + \frac{d(k-H)}{k} + \alpha^{-1} \left(1 - \frac{H}{k} + \frac{d(k-H)}{k}\right)$ on these bids. So we can't expect to get a very good upper bound on the fair value since the mechanism achieves a good lower bound. 

Suppose we consider a small finite number of bid types that within some power $\alpha^c$ where $\alpha$ is the bid ratio condition. Again, the above mechanism will achieve a fair value of $\frac{H}{k} + \frac{d(k-H)}{k} + \alpha^{-c} \left(1 - \frac{H}{k} + \frac{d(k-H)}{k}\right)$ on these bids. If we fix the bid ratio condition to be $\alpha = \left(\frac{1}{r}\right)^{1/c}$, then we can obtain a fair value of $r$ (this does not grow badly with $k$).

So, we will need to consider bids that are far apart in order to have any hope of proving good upper bounds. 

Maybe can we achieve better mechanisms? It's not obvious how to handle even discretized bids $\ldots , b^{-2}, b^{-1}, 1, b, b^2, \ldots $ with a uniform metric and total variation fairness. I'd like to apply some function where I give an extra mass of $\frac{d(k-1)}{k}$ to a bid if it increases by $\alpha^2$ and decrease all other bids by $\frac{d}{k}$ (i.e. $1, \ldots, 1$ (and $c, c, \ldots, c$ for all $c$) is given $\frac{1}{k}, \ldots, \frac{1}{k}$ and $\alpha^2, 1, \ldots, 1$ is given $\frac{1}{k} + \frac{d(k-1)}{k}, \frac{1}{k} - \frac{d}{k}, \ldots, \frac{1}{k}-\frac{d}{k}$.) While such a scheme may work for multiple task fairness, it will not work for total variation fairness (imagine $\alpha^2, \alpha^2, 1, \ldots, 1$; it will be given mass $\frac{1}{k} + \frac{d(k-1)}{k}, \frac{1}{k} + \frac{d(k-1)}{k}, \frac{1}{k} - \frac{d}{k} \ldots, \frac{1}{k}-\frac{d}{k}$ which violates total variation fairness.) Thus, it's not clear how to smoothly allocate the extra mass between the high-ish bids while handing arbitary jumps in bids. (We can't use the idea from before of evenly spreading it, but we also don't want to proportionally allocate...)

I don't know yet how to show a stronger upper bound either. 
